A Quantitative Study of Pure Parallel Processes

In this paper, we study the interleaving -- or pure merge -- operator that most often characterizes parallelism in concurrency theory. This operator is a principal cause of the so-called combinatorial explosion that makes very hard - at least from the point of view of computational complexity - the analysis of process behaviours e.g. by model-checking. The originality of our approach is to study this combinatorial explosion phenomenon on average, relying on advanced analytic combinatorics techniques. We study various measures that contribute to a better understanding of the process behaviours represented as plane rooted trees: the number of runs (corresponding to the width of the trees), the expected total size of the trees as well as their overall shape. Two practical outcomes of our quantitative study are also presented: (1) a linear-time algorithm to compute the probability of a concurrent run prefix, and (2) an efficient algorithm for uniform random sampling of concurrent runs. These provide interesting responses to the combinatorial explosion problem.

==> related.tex <==

%% related work


%%% Un mot spécial en hommage a flajolet qui déjà très tôt s'occupait
%%% de problèmes connexes.

The shuffle on trees can also be seen as a simplistic form of sequential scheduling,
finding admissible \emph{concurrent runs} based on precedence constraints. The latter corresponds
to tree-structured partial orders, thus
connecting our study to ordered set theory~\cite{BW91}, in particular to the problem of counting 
the \emph{linear extensions} of (tree-structured) partial orders (i.e. the set of
compatible total orders).


%%% counting linear extensions

Counting linear extensions of arbitrary Posets is $\sharp P$-complete~\cite{BW91}.
Tree-like partial orders represent a much simpler setting, and it is thus not surprising that efficient
 algorithms can be proposed in this favorable situation. Indeed, Atkinson proposes in~\cite{Atkinson90} a
 quadratic algorithm for couting the linear extensions of tree posets. This is to compare to our linear
 algorithm that is obtained by a direct implementation of the \emph{hook length} formula for couting
 increasing trees.  As it is often the case, the key element here is the natural bijection between
 increasing trees and the linear extensions of a tree poset.

%%% generating linear extensions

Compared to known algorithms for more general partial orders,
e.g.~\cite{DBLP:journals/dm/Huber06}, the proposed algorithm is much
simpler and efficient.
